Multi-View Bayesian Correlated Component Analysis

Correlated component analysis as proposed by Dmochowski et al. (2012) is a tool for investigating brain process similarity in the responses to multiple views of a given stimulus. Correlated components are identified under the assumption that the involved spatial networks are identical. Here we propose a hierarchical probabilistic model that can infer the level of universality in such multi-view data, from completely unrelated representations, corresponding to canonical correlation analysis, to identical representations as in correlated component analysis. This new model, which we denote Bayesian correlated component analysis, evaluates favourably against three relevant algorithms in simulated data. A well-established benchmark EEG dataset is used to further validate the new model and infer the variability of spatial representations across multiple subjects.

==> files/Auditory_Visual_EEG.tex <==
\section{Validation on benchmark EEG from an audio-visual selective attention task}
For the purpose of evaluating the algorithm on real EEG, a well-documented dataset from the Auditory-Visual Shift study by the renowned Swartz Center has been procured.
\subsection*{Experimental design}
The paradigm was designed to test the effect of ageing on neural responses of the auditory and visual stimuli. The auditory stimuli were 100-ms duration 550-Hz (target) and 500-Hz (non-target) sine-wave tones and the visual stimuli were light-blue (target) and dark-blue (non-target) filled squares presented for 100 ms on a light-grey background. During the experiment the subject was notified to either attend to visual or auditory stimuli and press a button when detecting a relevant target.
\subsection*{Pre-processing}
The continuous EEG was recorded from 33 channels of the international 10-20 system at 250 Hz from 49 subjects (5 discarded for missing events). The EEG was re-referenced to the left mastoid and segmented into response-locked epochs with 200 ms pre- and 900 ms post-response time. Epochs with values higher than 70$\mu V$ or exceeding 5 standard deviations were automatically rejected to remove eye artefacts and electrical drift. The remaining epochs were bandpass filtered using a windowed sinc-filter with passband frequencies 0.1-40 Hz and baseline-corrected in relation to the 200 ms pre-response interval. The "infomax" ICA algorithm \cite{Bell1995} was then used on the concatenated epochs to find the de-mixing matrix and isolate independent components containing eye artefacts. The "fully" automatic algorithm ADJUST \cite{Mognon2010} was used to identify noisy components which were then conservatively inspected manually and removed from the EEG. The EEG was then normalised with respect to its total power. 
\subsection*{Finding correlated components}
Because BCorrCA is sensitive to temporal misalignment the views used in this test was chosen based on the correlation between the averaged ERP of channel P3 for view 8 and the rest of the views. The six views with highest correlation (including self) were chosen and cropped to contain the same number of epochs (n=394). To test the reliability of the algorithm 100 epochs are randomly drawn from each view and concatenated to create 6 views of "continuous" EEG to be analysed in BCorrCA. The procedure is repeated 100 times in order to compute mean and standard error of the mean.
\subsection*{Results}
The variance of and difference between view-specific filters represents an estimate of the similarity between these. The same applies to the time series components but the algorithm only computes a common component for all the views, however, by constructing the backward model filters, \textbf{W}, the view-specific components can be found by $Z^{(m)} = W^{(m)} X^{(m)}$. In table \ref{tab:variance} we see that the average within-view variance for both filters and time series are significantly larger than the average between-view variance which suggests a high amount of universality in the neural representations. 
\begin{figure}
\begin{center}
\includegraphics[width=0.7\linewidth]{./pics/filter_projections_avg}
\end{center}
 \textbf{\refstepcounter{figure}\label{fig:filter_projections_avg} Figure \arabic{figure}.}{ Average filter projections over 10 repetitions }
\end{figure}
\begin{figure}
\begin{center}
\includegraphics[width=0.7\linewidth]{./pics/avg_comp_epoch}
\end{center}
 \textbf{\refstepcounter{figure}\label{fig:avg_comp_epoch} Figure \arabic{figure}.}{ Average ERP of component from BCorrCA and GFA }
\end{figure}
\begin{figure}
\begin{center}
	\includegraphics[width=0.7\linewidth]{./pics/filter_projection_3D}
\end{center}
 \textbf{\refstepcounter{figure}\label{fig:filter_projection_3D} Figure \arabic{figure}.}{ Grand average filter projection and standard error }

\end{figure}

\begin{table}
\renewcommand{\arraystretch}{1.3}
\textbf{\refstepcounter{table}\label{tab:variance} Table \arabic{table}.}{\small Variance of time series components and filters }
\processtable{ }{
	\begin{tabular}[C]{r|cc}
	 & Within-view & Between-view \\\hline %\vspace{5pt}
	Filters & 0.0456841 & 0.0184794\\
	Time series & 0.0949993 & 0.00998341
	\end{tabular}}{}
\end{table}


==> files/artif.tex <==
\begin{figure*}[!htb]
\centering
\begin{subfigure}[b]{0.48\linewidth}
	\includegraphics[width=\textwidth]{./pics/varSNR_K1_M2_L1000_normdata_sub}
	\caption{Two views}\label{fig.simsnr1}
\end{subfigure}
\hspace{2pt}
\begin{subfigure}[b]{0.48\linewidth}
	\includegraphics[width=\textwidth]{./pics/varSNR_K1_M5_L0_normdata_sub}
	\caption{Five views}\label{fig.simsnr4}
\end{subfigure}\\
%
%
\begin{subfigure}[b]{0.48\linewidth}
	\includegraphics[width=\textwidth]{./pics/varM_K1_SNRm6to6_l0_normdata_sub}
	\caption{Varying M}\label{fig.simm}
\end{subfigure}
\hspace{2pt}
\begin{subfigure}[b]{0.48\linewidth}
	\includegraphics[width=\textwidth]{./pics/varL_K1_M5_SNRm3to3_normdata_sub}
	\caption{$M=5$}\label{fig.siml}
\end{subfigure}
%\captionsetup{width=0.85\textwidth}
\caption{Performance of BCorrCA, GFA, CorrCA and CCA on simulated data measured by mean correlation coefficient and standard error of the mean with respect to the true source over 20 repetitions. In each subfigure the data is varied in one condition: In \textbf{(a)} and \textbf{(b)} the performance is tested under different levels of SNR and either 2 or 5 views. \textbf{(c)} shows the performance with varying number of views, and in \textbf{(d)} the similarity between the true weights are varied by the $\lambda$ parameter. Both data for both \textbf{(c)} and \textbf{(d)} are created with $\textnormal{SNR}=-6$. In all subfigures $\lambda=10^{-3}$, except for \textbf{(a)} where $\lambda=10^3$.} 
\label{fig.simres}
\end{figure*}

==> files/pcca.tex <==
\section{Probabilistic Correlated Component Analysis}
Inspired by the probabilistic principal component analysis introduced by \cite{tipping1999}, a probabilistic approach to CCA was presented in \cite{bach2005} using latent variables. They formulated a probabilistic generative model based on  Gaussian distributed common sources, \textbf{z}, mixed to form two noisy observed datasets;
\eq{
\mathbf{z} &\sim \mathcal{N}(\textbf{0},\mathbf{I}) \label{eq.zprior}\\
\textbf{x}^{(m)} &\sim \mathcal{N}\left(\textbf{A}^{(m)} \mathbf{z}, {\mathbf{\Phi}^{(m)}}\right)\quad  \textnormal{for}\ \, m = \{1,2\},
}
with $\mathbf{\Phi}^{(m)}$ representing the covariance matrix for the observation noise of dataset $m$. $\textbf{A}^{(m)} \in \mathbb{R}^{D\times K}$ signifies the mixing matrix%
%
\footnote{Authors use different letters for the mixing matrix. Most Bayesian models use the notation \textbf{W}, probably stemming from \cite{bishop1999}, but as this letter is also used to define the demixing matrix, we have in this article chosen to use \textbf{A} as employed in \cite{Parra2005}.}%
%
, where each of the $K$ columns represents the mixing of one source. To avoid discrete model selection in the related case of probabilistic PCA \cite{bishop1999} introduced automatic relevance determination (ARD), where each column in the mixing matrix has a Gaussian distribution and is regulated by a gamma distributed hyperparameter;
\eq{
\textbf{A}^{(m)} \sim \prod_k^K\mathcal{N}\left(\textbf{a}_k^{(m)}|\textbf{0}, \alpha^{-1}_k\right) \\
\boldsymbol\alpha \sim \prod_k^K\mathcal{G}a(\alpha_k|a_0,b_0).\label{eq.aprior}
}

These methods to probabilistic PCA and CCA has lead to different approaches to a Bayesian CCA e.g. \cite{Wang2007, Wu2011, klami2013} and group factor analysis (GFA) \cite{virtanen2011}, the first practical multi-view generalization of Bayesian CCA. The novelty in these methods were in how they approximated the posterior distribution for the hidden sources, using a full Bayesian treatment with many employing variational inference, as is also the case for the algorithm presented in this article.

Variational inference simplifies the posterior distributions by assuming that they are completely factorised (a method known in physics as \textit{mean field theory}). It uses the Kullback-Leibler (KL) divergence as a measure of the dissimilarity between the true distribution and its approximation, and seeks to minimise it.
The resulting algorithm consists of updating the lower bound with respect to each variable in turn in a expectation maximisation like manner. The way the updates are calculated makes exponential prior distributions a convenient choice, with the benefit of having conjugate relationship between the prior and posterior distributions \cite{Bishop2006, Murphy2012}.
